syGlass: Interactive Exploration of Multidimensional Images Using Virtual Reality Head-mounted Displays

The quest for deeper understanding of biological systems has driven the acquisition of increasingly larger multidimensional image datasets. Inspecting and manipulating data of this complexity is very challenging in traditional visualization systems. We developed syGlass, a software package capable of visualizing large scale volumetric data with inexpensive virtual reality head-mounted display technology. This allows leveraging stereoscopic vision to significantly improve perception of complex 3D structures, and provides immersive interaction with data directly in 3D. We accomplished this by developing highly optimized data flow and volume rendering pipelines, tested on datasets up to 16TB in size, as well as tools available in a virtual reality GUI to support advanced data exploration, annotation, and cataloguing.

==> syglasspaper-combining_dvr_and_meshes.tex <==
\subsection{Volumetric and Mesh Data Compositing}

Volume rendering utilities Ray Casting technique which produces a projection of volume data. This projection is used later as overlay when blended with previously rendered scene. This type of combining two scenes work for a general case, when the rest of scene is always behind the volume.

In the case of emission-only model, a natural way to blend two images is to use addition blend mode, since volume does not absorb light and should not reduce intensity of geometry behind. In the case of emission absorption model, a proper way to do the blending would be alpha composing. 

The image that is produced by DVR always has an alpha channel, which contains accumulated alpha value along the ray. To be able to use both optical models, pre-multiplied alpha composing is used. That means, that blending operation expects source values to be already multiplied by the alpha value. Thus it is possible to handle both models seamlessly. Emission-only model outputs the computed color and an always zero alpha, while emission-absorption model outputs pre-multiplied by the alpha color and an alpha value.

However, such a system will work only if all the scene is behind the volume, which is not true, since we need to render annotation geometry. Not handling this case leads to "impossible" images, which "breaks" stereoscopic vision. Objects that are in front of the volume are overlapped by it, the result is that it is hard to use such annotation tools in VR.

To render geometric scene with combination of volume rendering, was developed the following procedure:

\begin{itemize}
	\item First rendered the whole geometric scene, saving the depth buffer to a texture.
	\item Then content of the texture with depth information is rendered to a second framebuffer attached to a float-point texture. At this step, the mapped depth information is transformed to actual distance from camera to the fragment and also wrapped to match the wrapped space in which the volume is rendered.
	\item At ray-casting step, the rendered at previous step texture is used. All rays that cross the distance stored in the texture corresponding to given ray are terminated, because they are treaded as rays that encountered an opaque surface.
	\item As a last step, a regular blending is performed, that was described earlier.
\end{itemize}


\begin{figure}[htbp]
\begin{tabular}{cc}
\subfloat[]{\includegraphics[width=1.6in]{dvr_depth}} & \subfloat[]{\includegraphics[width=1.6in]{dvr_wrapped}} \\
\subfloat[]{\includegraphics[width=1.6in]{dvr_mesh}} & \subfloat[]{\includegraphics[width=1.6in]{dvr_unwrapped}} \\
\end{tabular} 
\subfloat[]{\includegraphics[width=3.5in]{dvr_final}}
\caption{\textbf{Volume rendering.} a) Wrapped depth buffer; b) Result of DVR in wrapped space, with depth buffer; c) Previousle rendered mesh scene, which was the source of depth information; d) Mesh scene combined with unwrapped DVR buffer; e) Final image with applied barrel distortion to compensate lenses distortion.}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "syglasspaper-main"
%%% End:


==> syglasspaper-imposters.tex <==
\subsection{Imposters}

\begin{itemize}
  \item  Rendering of annotation data
  \item  Why imposters? Dynamically modified data
  \item  Effeciency of imposters
  \item  How imposters work
  \item  Geometry shaders
  \item  Primitives: sphere and cone
  \item  Detailed description for sphere case
  \item  Contraction of cage for cone
\end{itemize}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "syglasspaper-main"
%%% End:


==> syglasspaper-octree.tex <==
\subsection{Octree Representation}

All volumetric data is stored and rendered as octrees. Octree structure allows storing a multi-resolution pyramid. The goal is to select levels of resolution of the pyramid, so that pixel resolution of the rendered images matches the angular resolution of the voxels currently traversed. Octree structure allows us to maintain a constant amount of voxels sampled per frame, that significantly lowers the amount of memory and computational resources needed to render the frame.
Utilizing octree representations of volumes, we have built a system that was proven to visualize datasets of size up to 16TB.


To enable large scale volumetric rendering a visualization-driven approach was implemented, so that only required data is loaded and rendered. In many cases datasets are significantly larger than on-board GPU memory and can reach hundreds of terabytes. Our system was successfully tested with 16TB dataset and have shown good performance for VR. The system can scale to large data by performing visualization and computation tasks proportional to the currently visible data, required data sampling frequency and ray density. To perform needed visualization, size of working set is fixed that allows to scale to large volumes.

We use an octree-based multi-pass render to make the visualization pipeline scalable. Tree traversal happens on the CPU, during which a schedule of blocks to be rendered is created. Each block is rendered using a separate draw call. All the blocks are sorted and rendered from the front to the back block that guarantees correct integration for the emission-absorption model and allows early ray termination. All the blocks are rendered to the intermediate framebuffer with color and alpha channels in the wrapped space. When a subsequent block is rendered, the ray is continued inside that block by reading previously written values of color and alpha. After the ray reaches the end of current block or has terminated, new values of color and alpha are written back.

The tree traversal algorithm starts from the root node and then checks if the current resolution level is enough or no. If it suits, then the current block is registered in the render list. If not, the procedure repeats recursively for all children nodes. Children nodes are traversed in the order that matches the overlapping order, thus the resulting render-list appears to be sorted from the front to the back block. The traversal algorithm also performs frustum culling of the blocks by ignoring not visible ones. The decision on if the current resolution level suits the needs of creating a quality rendering for the user or not is taken by comparing the needed angular voxel resolution with angular resolution provided by the block by it's closest face at the given distance.

If one or more of the children blocks are currently not in the cache, they are added to the request queue and a resolution one level above is used. When the all children blocks are loaded, the the needed resolution level is used.

Each time a block is used, it's time-stamp is updated. The time-stamp is used by the two level cache system which consists of block cache at the on-board GPU memory and block cache at CPU RAM. Both caches are using priority queues to unload blocks with the oldest timestamps. 

\begin{figure}[htbp]
\centering
\begin{tabular}{ccc}
\subfloat[]{\includegraphics[width=1.0in]{octree_first_pass}} & \subfloat[]{\includegraphics[width=1.0in]{octree_half}} & \subfloat[]{\includegraphics[width=1.0in]{octree_warped}} \\
\end{tabular} 
\subfloat[]{\includegraphics[width=2.5in]{octree_final}}
\caption{\textbf{Octree multipass rendering.} a) Result of the first pass; b) Accumulated image after half of all passes were completed; c) Result after all passes were done; d) Unwrapped image.}
\end{figure}


\begin{figure}[th!]
\centering
\includegraphics[height=2.0in]{20170611022854}
\caption{\textbf{Octree based visualization.} Leafs of the octree are marked with white bounding boxes.}
\label{fig:octree}
\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "syglasspaper-main"
%%% End:


==> syglasspaper-warping.tex <==
\subsection{Optimising DVR for VR}

One of the problems that arises when a computationally incentive rendering is needed for VR is large field of view. Large field of view is needed because of peripheral vision. However, because of the distortion introduced by VR driver to compensate the distortion of the lenses, all peripheral area of the image gets downsampled. In addition, human vision at peripheral region has much lower resolution. As a result, a natural approach to optimize volume rendering for VR would be to vary ray density across the image.

We implemented a DVR system that renders volume in wrapped space with uniform ray distribution to an image. Then the image is unwrapped to the original space in which space ray distribution becomes non uniform. 

Without applying the wrapping, to cast a ray from a given pixel, it's coordinates should be reverse projected to get the ray direction. To apply the wrapping an additional map is used to transform the coordinates to a new position before reverse projection is made. After the image is rendered, an inverse mapping is used to unwrap the image.

This technique allows significantly lower amount of the rays and thus improves volume rendering performance for VR without noticeable degradation in image quality.


\subsection{3D Movies}

We have implemented playing of movies, that are sequences of volumetric frames. Volumes of small size, such as less then $20x10^6$ total voxels, can played at a high frame-rate (25FPS). That is achieved by storing data compressed with LZ4, as described earlier in section \ref{container}, that stores data already memory aligned therefore no additional manipulations are required to upload the data to the GPU after decompression. 

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "syglasspaper-main"
%%% End:

